Image Clustering using an Augmented Generative Adversarial Network and Information Maximization

Image clustering has recently attracted significant attention due to the increased availability of unlabelled datasets. The efficiency of traditional clustering algorithms heavily depends on the distance functions used and the dimensionality of the features. Therefore, performance degradation is often observed when tackling either unprocessed images or high-dimensional features extracted from processed images. To deal with these challenges, we propose a deep clustering framework consisting of a modified generative adversarial network (GAN) and an auxiliary classifier. The modification employs Sobel operations prior to the discriminator of the GAN to enhance the separability of the learned features. The discriminator is then leveraged to generate representations as the input to an auxiliary classifier. An adaptive objective function is utilised to train the auxiliary classifier for clustering the representations, aiming to increase the robustness by minimizing the divergence of multiple representations generated by the discriminator. The auxiliary classifier is implemented with a group of multiple cluster-heads, where a tolerance hyper-parameter is used to tackle imbalanced data. Our results indicate that the proposed method significantly outperforms state-of-the-art clustering methods on CIFAR-10 and CIFAR-100, and is competitive on the STL10 and MNIST datasets.

==> includes/auxiliary_classifier_old.tex <==
\subsection{Auxiliary Classifier}

Further to the above architecture, we train an auxiliary network explicitly on top of the discriminator to classify the extracted features of the discriminator model. Our clustering strategy is based on IMSAT \cite{Hu2017} which implements RIM \cite{Gomes2010}.

Before explaining the training process, we briefly describe the mutual information to be applied in RIM \cite{Gomes2010}, which is defined as follows:
\begin{dmath}
I(X;Y) = H(Y) - H(Y|X)
\label{eq:MI}
\end{dmath}

The conditional entropy on the right hand side can be rewritten as:

\begin{dmath}
H(Y|X) = \frac{1}{N}\sum_{i=1}^N{H\{p(y|x_i,W)\}} 
\label{eq:conditional}
\end{dmath}

% \[\begin{array} {lcl}H(Y|X) & = &  \frac{1}{N}\sum_{i=1}^N{H\{p(y|x_i,W)\}}
% \\ & = & \frac{1}{N}\sum_{i=1}^N{-p(y,x_i)*log(p(y|x_i,W))}
%\end{array}\]
        
where Shannon entropy (hence the conditional entropy term \ref{eq:conditional}) strictly satisfies $H(Y|X) \geq 0$. Therefore, minimizing the conditional entropy penalizes the model to assign a high probability to the relevant clustering index, since the uncertainty is diminished. The marginal entropy term of the right hand side is expressed by: 

\begin{dmath}
H(Y) = H\{\frac{1}{N}\sum_{i=1}^N{p(y_i|W)\}} 
\label{eq:marginal}
%H(Y) = \frac{1}{N}\sum_{i=1}^N{H\{p(y|W)\}} 
\end{dmath}

according to the information theory \cite{Cover:1991:EIT:129837}, the marginal entropy follows the upper bound $H(Y)\leq log(k)$. By maximizing the marginal entropy ($H(X) \approx log(k)$), the model is forced to evenly distribute the class thresholds (increasing the uncertainty), \textbf{Please reformulate the following sentence}
%for instance an ideal scenario such as that of perfect class distributed dataset. Therefore, by applying the aforementioned rules, we have  \cite{Cover:1991:EIT:129837}:
%we show how the model evenly distributes the class thresholds.
where this occurs in a perfect balanced dataset as the model is penalised of assigning the class indices uniformly. Therefore, by applying the aforementioned rules, we have  \cite{Cover:1991:EIT:129837}:
%In an ideal scenario - such as that of a perfect balanced dataset - the highest value of this quantity is equal to $log(k)$. According to information theory \cite{Cover:1991:EIT:129837}:

\begin{dmath}
D_{KL}(p||u) = \sum p(x)log \frac{p(x)}{u(x)} = log(k) - H(X)
\label{eq:equality}
\end{dmath}

where $u$ is a uniformly distributed prior. Thence, according to eq. \ref{eq:equality}, maximizing $H(Y)$ is similar to minimizing any the term in eq \ref{eq:equality}. Here, we combine the two parts of conditional entropy and described equality term in order to transform the above two functions (\ref{eq:conditional},\ref{eq:marginal}) to obtain strictly positive values. Consequently, we aim to minimize the following term as the RIM part of the objective function \cite{Hu2017}.

\begin{dmath}
max([D_{KL}(p||u)  - \delta],0) + H(Y|X)
\label{eq:minimize entropy}
\end{dmath}

where $\delta \geq 0$ denotes an introduced tolerance factor which encourages the model's cluster distribution $p_{\theta}(y)$ to approximate the uniform prior within a defined tolerant level. The application of $\delta-$tolerant increases the model's avoidance of producing degenerate solutions; as without it, the model will be forced to balance the training samples equally hence resulting to assign trivial solutions in the case of non-balanced datasets. We found that optimizing the model's parameters by performing gradient descent where a tolerance factor is introduced, the model results to higher capability in term of accuracy based on experiments presented in sub-section \ref{sub:auxiliary classifier}. \par
In the following, we turn to penalising the corresponding function in the IMSAT case by borrowing the idea in the Self-Augmented Training (SAT) \cite{Hu2017} approach. In SAT, the penalty term can be described mathematically as follows \cite{Hu2017}:
\begin{dmath}
R_{SAT}(\theta;T) = \frac{1}{N}\sum_{n=1}^N{R_{SAT}(\theta;x_n,T(x_n))}
\end{dmath}

where $T(x) = x + r$ denotes a transformed function with input $x$ and a perturbation $r$. The above regularized function is expressed with the application of Kullback–Leibler divergence (KL), and theoretically the original version of $x$ and the transformation should have the same distribution in the probabilistic layer. Therefore, diminishing the KL divergence will make our network to equally distribute the two inputted samples (original, transformed). Two alternative methodologies, Random Perturbation Training (RPT) and Virtual Adversarial Training (VAT) are proposed in IMSAT. In this work, we make use of the VAT regularization which has perturbation $r$ as an adversarial direction \cite{Miyato2017VirtualAT}:

\begin{equation}
 %\begin{split}
    L_{adv}(x,\theta)=D_{KL}(p(y|x,\theta),p(y|x+r_{adv},\theta) 
\end{equation}
\begin{equation}
\text{where } r_{adv} := \underset{r;\|r\|^2 \leq \epsilon}{argmax}\{D_{KL}(p(y|x,\theta),p(y|x+r,\theta)\}
%\end{split}
\label{eq:epsilon}
\end{equation}

Similar to \cite{Miyato2017VirtualAT}, we approximate $r_{adv}$ based on the $L_2$ norm, which can be expressed as $r_{adv} \approx e \frac{g}{\|g\|^2}$, where $g$ denotes the computed gradient with respect of the relevant point. In this work, $y$ is a probabilistic output of the softmax distribution function. In addition, we make use of multiple cluster heads (softmax layers), \textbf{Rewrite the following sentence} where the complete version of our clustering functions is derived as:
%which when combined denotes the complete version of our clustering function as:


\begin{equation}
\begin{split}
L (\theta;m,m+r') &= \frac{1}{L}\sum_{j=1}^L \frac{1}{N}\sum_{n=1}^N\{{R_{SAT}(\theta;m_n,T(m_n))}
\\ &+ \lambda[max([D_{KL}(p||u)  - \delta],0)
\\ &+ H(Y|M)]\}
\end{split}
\label{eq:function_complete}
\end{equation}

where $L$ denotes the number of cluster heads, $\lambda$ a weight parameter and $M$ the new domain space produced by the discriminator model. 
%Through the multiple cluster heads, we encourage the model to assign sensible solutions {\textbf{What does this exactly mean?}}. 
Through the multiple cluster heads, the model is encouraged of increasing the prediction accuracy by assigning more sensible solutions {\textbf{What does this exactly mean? - i changed a bit the sentence, based on the experiments that i performed, it seems that through the multiple cluster-heads the classifier increases the prediction accuracy}}. 
This occurs since the probabilistic outputs are optimized simultaneously and the cluster head with a lower loss guides the heads with the higher loss performance (further details in table \ref{tab: effects cluster-heads}). We also vary the value of $k$ to a higher range than its predefined value through an additional cluster head, in order to capture more details such as variations or sub-classes, within similar classes. \par 
Through this combination of varying $k$ with multiple cluster layers, our experiments have shown that this approach (multiple cluster heads) increases the model's predictive capability/accuracy. In the case of a high $k$ value, delta ($\delta$) is initialised with a higher value, since we made the assumption that training samples within sub-classes are not evenly distributed. The results and effects of different parameters' values are presented in the following section.\par

\SetKwInOut{Initialize}{Initialize}
\SetKwInOut{Generate}{Generate}

\begin{algorithm}[htb]
\KwData{$X=\{x_{i}\}_{i=1}^{n}$}
\Initialize{$(G_\theta,D_\theta,Aux_\theta)$ }
\While{Converge condition}{
  \hspace{0.7mm} \textbullet \hspace{0.1mm} Sample $n$ elements $\{x^{(1)},...,x^{(n)}\}$ \\
 \textbullet \hspace{0.1mm} Sample random minibatch $z_n \in [-1,1]$\\
\textbullet \hspace{0.1mm} Update the discriminator by ascending: \\
$\vcenter{
  \begin{align*}
  \nabla_{D_\theta} \frac{1}{n}\sum_{i=1}^{n}[log(D(x_i))+log(1-D(G(z_i)))]
 \end{align*}
 }$
  \textbullet \hspace{0.1mm} Sample random minibatch $z_m \in [-1,1]$\\
  \textbullet \hspace{0.1mm} Update the generator by ascending: \\
  $\vcenter{
  \begin{align*}
  \nabla_{G_\theta} \frac{1}{n}\sum_{i=1}^{n}[log(D(G(z_i)))]
 \end{align*}
 }$
}
%\Initialize{$Aux_\theta$}
\Generate{$D(X) \rightarrow M$}
\While{Converge condition}{
  \hspace{0.7mm} \textbullet \hspace{0.1mm} Sample $n$ features $\{m^{(1)},...,m^{(n)}\}$ \\
  \textbullet \hspace{0.1mm} Update the auxiliary classifier by ascending: \\
\begin{align*}
\begin{split}
\nabla_{Aux_\theta} &= \frac{1}{L}\sum_{j=1}^L \frac{1}{N}\sum_{n=1}^N\{{R_{SAT}(\theta;m_n,T(m_n))}
\\ &+ \lambda[max([D_{KL}(p||u)  - \delta],0)
\\ &+ H(Y|M)]\}
\end{split}
\end{align*}

}
\caption{Proposed clustering process}
\label{alg:Process}
\end{algorithm}

Algorithm \ref{alg:Process} describes in detail the complete training process comprised of two consecutive phases. Note that at no stage do the proposed framework require any labels for the data when training our model.

%In contrast to the original proposal in \cite{Miyato2017VirtualAT}, we replace the initial perturbation $r$ as described in eq. \ref{eq:epsilon} with the operation of dropout operation within the hidden layers. Hence, we avoid of generating random noise which in circumstances pre-knowledge of $p(x)$ is required of appropriately defining value of $\epsilon$ in early stage. 

%It performs transformation implicitly through the discriminator model. Our discriminator network is trained with the implication of drop out layer, therefore the initial content of the image remain invariant but the generated vectors are transformed based on drop rate that is set.  



%For computing the adversarial perturbation ($m+r_{adv}$), two steps are carried out as follows. Firstly, as shown in eq. \ref{eq:epsilon} we compute the initial gradient in respect to the classifier's input and KL diverge, where both $y$'s are computed parallel with drop rate to set $0\%$ and $50\%$ respectively, and without additional noise to be generated. In the second phase, the generated gradient is normalized based on $L_2$, normalised based on $e$ factor and combined with the extracted features for the second round as derived from VAT. Further details for adversarial training are provided in \cite{Miyato2017VirtualAT,miyato2015distributional}. Lastly, subject to $r_{adv};\|r_{adv}\|^2 \leq e$, we adapt the scale factor individually based on $e_i=0.15*||m_i||^2$, where $i$ denotes $i_{th}$ element in training batch.

%For computing the adversarial transformation ($m+r_{adv}$), two steps are to be carried out as follows. Firstly, $r$ is computed from a normal distribution and normalized by an $L_2$ norm $r = e \frac{r}{\|r\|^2}$, where $r$ denotes the random sample and $e$ is derived from eq. \ref{eq:epsilon} and set to $10$ for random perturbations. The transformed versions and original features are passed to the model as training data \textbf{What does 'forwarded' mean here? - change to pushed forward}. In the second step, the generated gradient is computed with respect to the input $M$ using a back propagation process. Further details for adversarial training are provided in \cite{Miyato2017VirtualAT,miyato2015distributional}. Additionally, subject to $r_{adv};\|r_{adv}\|^2 \leq e$, we defined $e=5$ across the experiments for CIFAR-10/100 and STL, since the generated $M$ features are weighted outside of the aforementioned {\bf state the interval to avoid ambiguity} interval. In the MNIST experiments, $e$ is set to $2.5$ due to the smaller variation within the produced features. Lastly, the virtual adversarial transformation is propagated forwarded \textbf{?? - changed to propagate forward} to the model in the final round. {\bf i would avoid phrases like pushed forward as they are not co clear. augmenting the data during training, or construction mini batches of the original and perturbed data would be clearer. I would also reduce the number fo ways you refer to it, currently you have transformed data, VAT data, etc. maybe use the term perturbation or augmentation and state that these are from VAT, is this done multiple times? its reads as if it is.}\par


%For computing the adversarial transformation ($m+r_{adv}$), two steps are to be carried out as follows. Firstly, $r$ is computed from a normal distribution and normalized by an $L_2$ norm $r = e \frac{r}{\|r\|^2}$, where $r$ denotes the random sample and $e$ is derived from eq. \ref{eq:epsilon} and set to $10$ for random perturbations. The transformed versions and original features are passed to the model as training data \textbf{What does 'forwarded' mean here? - change to pushed forward}. In the second step, the generated gradient is computed with respect to the input $M$ using a back propagation process. Further details for adversarial training are provided in \cite{Miyato2017VirtualAT,miyato2015distributional}. Additionally, subject to $r_{adv};\|r_{adv}\|^2 \leq e$, we defined $e=5$ across the experiments for CIFAR-10/100 and STL, since the generated $M$ features are weighted outside of the aforementioned {\bf state the interval to avoid ambiguity} interval. In the MNIST experiments, $e$ is set to $2.5$ due to the smaller variation within the produced features. Lastly, the virtual adversarial transformation is propagated forwarded \textbf{?? - changed to propagate forward} to the model in the final round. {\bf i would avoid phrases like pushed forward as they are not co clear. augmenting the data during training, or construction mini batches of the original and perturbed data would be clearer. I would also reduce the number fo ways you refer to it, currently you have transformed data, VAT data, etc. maybe use the term perturbation or augmentation and state that these are from VAT, is this done multiple times? its reads as if it is.}\par





%For computing the adversarial transformation ($m+r_{adv}$), two steps are to be carried out as follows. Firstly, $r$ is computed from a normal distribution and normalized as $r = e \frac{r}{\|r\|^2}$, where $e$ is a scale factor derived from eq. \ref{eq:epsilon}. We adapt $e$ proportion to the norm of each generated representation as $e_i = \alpha \cdot \|m_i\|^2$. We set $\alpha$ for experiments: CIFAR 10/100, STL to $0.3$ and MNIST to $2$ respectively. In the second round of VAT process, we define scalar as previously, where $a$ holds $0.15$ for the three grouped mentioned training sets and $0.5$ for MNIST. Further details for adversarial training are provided in \cite{Miyato2017VirtualAT,miyato2015distributional}.

